Why We Refactor? Confessions of GitHub Contributors

Refactoring is a widespread practice that helps developers to improve the maintainability and readability of their code. However, there is a limited number of studies empirically investigating the actual motivations behind specific refactoring operations applied by developers. To fill this gap, we monitored Java projects hosted on GitHub to detect recently applied refactorings, and asked the developers to ex- plain the reasons behind their decision to refactor the code. By applying thematic analysis on the collected responses, we compiled a catalogue of 44 distinct motivations for 12 well-known refactoring types. We found that refactoring activity is mainly driven by changes in the requirements and much less by code smells. Extract Method is the most versatile refactoring operation serving 11 different purposes. Finally, we found evidence that the IDE used by the developers affects the adoption of automated refactoring tools.

==> tbl/TabIntellijDevelopers.tex <==
\begin{tabular}{@{}lrlrl@{}} \toprule
Group & \multicolumn{2}{c}{Occurrences} & \multicolumn{2}{c@{}}{Automated \%} \\ \midrule
IntelliJ IDEA Developers & 11 & \sbar{11}{40} & 73\% & \sbar{8}{11} \\
IntelliJ IDEA Users & 40 & \sbar{40}{40} & 70\% & \sbar{28}{40} \\
%Other IDE Users & 30 & \sbar{30}{40} & 43\% & \sbar{13}{30} \\
\bottomrule \end{tabular}

==> tbl/TabMoveClassMotivations.tex <==
\begin{tabular}{@{}p{0.25\linewidth}p{0.5\linewidth}rl@{}} \toprule
Theme & Description & \multicolumn{2}{c@{}}{Occurrences}\\ \midrule
Rename package & All classes from a package are moved to a new one, resulting in the same package but with a more appropriate name. & 13 & \sbar{13}{13} \\
Move class to more appropriate container & Class is moved to package that is more functionally/conceptually related to it. & 13 & \sbar{13}{13} \\
Introduce sub-package & Move one or more classes to form a new subpackage containing related packages. & 6 & \sbar{6}{13} \\
Convert to top-level container & Convert an inner class into a top-level class to widen its scope. & 4 & \sbar{4}{13} \\
Remove inner classes from deprecated container & Move an inner class out of a class that is beeing deprecated or removed. & 2 & \sbar{2}{13} \\
Remove from public API & Class is moved out of a package that contains external API to an internal package of the system, avoiding its unnecessary exposure. & 2 & \sbar{2}{13} \\
Convert to inner class & Convert a top-level class into an inner class to reduce its scope. & 2 & \sbar{2}{13} \\
Isolate dependencies & Move a class to another package to elliminate undesired dependencies between modules. & 1 & \sbar{1}{13} \\
Backward compatibility & Move class back to its original package to restore backward compatibility. & 1 & \sbar{1}{13} \\
\bottomrule \end{tabular}

==> tbl/TabRefactoringActivityProject.tex <==
\begin{tabular}{@{}lrr@{}} \toprule
Project & Commits  & Ref. types\\ \midrule
{\sc JetBrains/intellij-community} & 37 & 9 \\
{\sc facebook/buck} & 17 & 6 \\
{\sc apache/hive} & 15 & 3 \\
{\sc neo4j/neo4j} & 15 & 7 \\
{\sc apache/cassandra} & 14 & 4 \\
{\sc gradle/gradle} & 13 & 9 \\
{\sc VoltDB/voltdb} & 13 & 5 \\
{\sc CyanogenMod/android_fra\ldots} & 11 & 4 \\
{\sc hazelcast/hazelcast} & 10 & 7 \\
{\sc SonarSource/sonarqube} & 10 & 6 \\
\bottomrule \end{tabular}
